Efficient Near-Optimal Algorithm for Online Shortest Paths in Directed Acyclic Graphs with Bandit Feedback Against Adaptive Adversaries

In this paper, we study the online shortest path problem in directed acyclic graphs (DAGs) under bandit feedback against an adaptive adversary. Given a DAG $G = (V, E)$ with a source node $v_{\mathsf{s}}$ and a sink node $v_{\mathsf{t}}$, let $X \subseteq \{0,1\}^{|E|}$ denote the set of all paths from $v_{\mathsf{s}}$ to $v_{\mathsf{t}}$. At each round $t$, we select a path $\mathbf{x}_t \in X$ and receive bandit feedback on our loss $\langle \mathbf{x}_t, \mathbf{y}_t \rangle \in [-1,1]$, where $\mathbf{y}_t$ is an adversarially chosen loss vector. Our goal is to minimize regret with respect to the best path in hindsight over $T$ rounds. We propose the first computationally efficient algorithm to achieve a near-minimax optimal regret bound of $\tilde O(\sqrt{|E|T\log |X|})$ with high probability against any adaptive adversary, where $\tilde O(\cdot)$ hides logarithmic factors in the number of edges $|E|$. Our algorithm leverages a novel loss estimator and a centroid-based decomposition in a nontrivial manner to attain this regret bound. As an application, we show that our algorithm for DAGs provides state-of-the-art efficient algorithms for $m$-sets, extensive-form games, the Colonel Blotto game, shortest walks in directed graphs, hypercubes, and multi-task multi-armed bandits, achieving improved high-probability regret guarantees in all these settings.

==> extra.tex <==
 Let $\mathbb{E}_{t}[\cdot]=\mathbb{E}[\cdot|\calF_{t-1}]$ where $\calF_{t-1}$ is the past filtration. Similarly, let $\mathbb{P}_t(\cdot)=\mathbb{P}(\cdot|\calF_{t-1})$ denote the probability law in round $t$. It is easy to observe that for vertex $v\in E\cup V\setminus\{\source,\sink\}$, we have $\mathbb{P}_t(\bfx_t[v] = 1)=\tilde \bfx_t[v]$. We define our loss estimator $\widehat{\bfy}_t$ as follows: for each vertex $v \in V$, we set $\widehat{\bfy}_t[v] := \frac{\ind(\bfx_t[v] = 1) - \ind(\bfx_t[v] = 1)\ell_t}{\mathbb{P}_t(\bfx_t[v] = 1)}$, and for each edge $e \in E$, we define $\widehat{\bfy}_t[e] := \frac{\ind(\bfx_t[e] = 1) + \ind(\bfx_t[e] = 1)\ell_t}{\mathbb{P}_t(\bfx_t[e] = 1)}$.  It is important to note that our loss estimator $\widehat{\bfy}_t$ is not an unbiased estimator of $\bfy_t$. However, we claim that for any $\bfx, \bfx' \in \calX$, it holds that $\mathbb{E}_t[\langle \bfx - \bfx', \widehat{\bfy}_t \rangle] = \langle \bfx - \bfx', \bfy_t \rangle$. This property is sufficient for applying the standard analysis of Follow The Regularized Leader (FTRL).





\begin{proof}    
\todo[Zhiyuan]{Proof of Theorem~\ref{thm:equal-path-length-regret}}
We select $F(x) = -\sum\limits_{v \in V \setminus \{\source, \sink\}} \sqrt{x[v]} - \sum\limits_{e \in E} \sqrt{x[e]}$ as our regularizer. Applying the standard FTRL analysis, we show that the regret is $\calO(\sqrt{K |E| T})$. Since $\calX$ is finite and $F(x)$ is Legendre, there exists a unique minimizer $\tilde{\bfx}_t$ in each round $t$, with every coordinate of $\tilde{\bfx}_t$ strictly positive. By following the standard FTRL analysis from \citet{lattimore2020bandit}, we obtain the following:
\begin{equation*}
    \mathrm{Reg}(T)\leq \frac{\operatorname{diam}_F(\operatorname{co}(\calX))}{\eta}+\mathbb{E}\left[\sum_{t=1}^T\langle \tilde \bfx_t-\tilde \bfx_{t+1},\widehat \bfy_t\rangle-\frac{D_F(\tilde \bfx_t,\tilde \bfx_{t+1})}{\eta}\right]
\end{equation*}
First we upper bound $\sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{x[v]}+\sum\limits_{e\in E}\sqrt{x[e]}$ for any $x\in\operatorname{co}(\calX)$ as follows:
\begin{align*}
    \sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{x[v]}+\sum\limits_{e\in E}\sqrt{x[e]}&\leq \sqrt{(|V|+|E|-2)\cdot (\sum\limits_{v\in V\setminus \{\source,\sink\}}x[v]+\sum\limits_{e\in E}x[e])} \tag{Cauchy-Schwarz inequality}\\
    &\leq\sqrt{(2|E|)\cdot (\sum\limits_{v\in V\setminus \{\source,\sink\}}x[v]+\sum\limits_{e\in E}x[e])} \tag{as $|V|\leq |E|+1$}\\
    &\leq \sqrt{4K|E|}
\end{align*}
We get the last inequality due to the following. First by definition any point in $x\in\operatorname{co}(\calX)$ is a convex combination of points in $\calX$. Therefore for any $x'\in \calX$, an upper bound on $\sum\limits_{v\in V\setminus \{\source,\sink\}}x'[v]+\sum\limits_{e\in E}x'[e]$ is also an upper bound on $\sum\limits_{v\in V\setminus \{\source,\sink\}}x[v]+\sum\limits_{e\in E}x[e]$. As any path in the DAG $G$ has exactly $K$ edges, we have $\sum\limits_{v\in V\setminus \{\source,\sink\}}x'[v]=K-2$ and $\sum\limits_{e\in E}x'[e]=K$.

\noindent
Now we upper bound the diameter as follows:
\begin{equation*}
    \operatorname{diam}_F(\operatorname{co}(\calX))\leq \max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{x[v]}+\sum\limits_{e\in E}\sqrt{x[e]}\leq \sqrt{4K|E|}
\end{equation*}

Next, we upper bound the second term of the regret upper bound above. Let $\bfy_t'$ be a vector such that for all $i\in E\cup V\setminus\{\source,\sink\}$, we have $\bfy_t'[i]=\widehat\bfy_t[i]\ind\{\tilde \bfx_{t+1}[i]\leq \tilde \bfx_{t}[i]\}$. Since all the coordinates of $\widehat\bfy_t[i]$ are non-negative, we have the following:
\begin{equation*}
    \sum_{t=1}^T\langle \tilde \bfx_t-\tilde \bfx_{t+1},\widehat \bfy_t\rangle-\frac{D_F(\tilde \bfx_t,\tilde \bfx_{t+1})}{\eta}\leq \sum_{t=1}^T\langle \tilde \bfx_t-\tilde \bfx_{t+1},\bfy_t'\rangle-\frac{D_F(\tilde \bfx_t,\tilde \bfx_{t+1})}{\eta}\leq \frac{\eta}{2}||\bfy_t'||_{\nabla^2F(z_t)^{-1}}^2
\end{equation*}
where $z_t$ is some point on the chord $[\tilde \bfx_t,\tilde \bfx_{t+1}]$ and the last inequality follows from Lemma XYZ. Next observe that $\nabla^2F(z)=\operatorname{diag}(1/z^{3/2})$. Due to the definition of $\bfy_t'$, it follows that the term $||\bfy_t'||_{\nabla^2F(z_t)^{-1}}^2$ is maximized when $z_t=\tilde \bfx_t$. Hence, we have $\mathbb{E}\left[||\bfy_t'||_{\nabla^2F(z_t)^{-1}}^2|\calF_{t-1}\right]\leq 4\sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{\tilde \bfx_t[v]}+4\sum\limits_{e\in E}\sqrt{\tilde\bfx_t[e]}\leq 8\sqrt{K|E|}$. Hence, we have the following:
\begin{equation*}
     \mathrm{Reg}(T)\leq \frac{\operatorname{diam}_F(\operatorname{co}(\calX))}{\eta}+\mathbb{E}\left[\sum_{t=1}^T\langle \tilde \bfx_t-\tilde \bfx_{t+1},\widehat \bfy_t\rangle-\frac{D_F(\tilde \bfx_t,\tilde \bfx_{t+1})}{\eta}\right]\leq \frac{\sqrt{4K|E|}}{\eta}+\frac{8T\eta}{2}\sqrt{K|E|}\leq 4\sqrt{K|E|T}
\end{equation*}
where we get the last inequality by setting $\eta=\frac{1}{\sqrt{T}}$.

\todo{Recheck all the calculations.}
\end{proof}


==> pseudo.tex <==
\subsection{Refined pseudo-regret guarantees}\label{sec:refined-guarantees}
\todo[Arnab]{This pseudo-regret guarantee is not that important. Will work on it if time permits.}
For our FTRL approach in \Cref{sec:alg-make-equal}, we provide a refined regret guarantee based on the input DAG $G=(V,E)$. Let $\calX_{G}\subseteq\{0,1\}^{|E|}$ be the collection of all paths in $G$ indexed by the edges in $E$. Let $\calC^\star:=\max_{x\in\operatorname{co}(\calX_G)}\sum_{e\in E}\sqrt{x[e]}$. We now show that the regret of our FTRL approach is upper bounded by $\calO(\calC^\star\sqrt{T})$. 

Let $\calX$ represent the set of all paths $p$, including their appended bits. Let $\calD^\star:=\max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{x[v]}+\sum\limits_{e\in E}\sqrt{x[e]}+\sum\limits_{i=1}^{K-1}\sqrt{x[\ell+i]}$, where $\ell=|V|+|E|-2$. It follows easily from our analysis in the previous section that the regret is upper bounded by $\calO(\calD^\star\sqrt{T})$. Hence, it suffices to show that $\calD^\star\leq c\cdot \calC^\star$ where $c$ is some absolute constant.

First observe that $\max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{i=1}^{K-1}\sqrt{x[\ell+i]}\leq K-1$. Next, consider a path $x\in \calX$ of length $K$. Observe that $\sum_{e\in E}\sqrt{x[e]}=K$. Hence, $\max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{i=1}^{K-1}\sqrt{x[\ell+i]}\leq\max\limits_{x\in \operatorname{co}(\calX)}\sqrt{x[e]} $. Next, consider $x\in \operatorname{co}(\calX)$. Let $\delta^{-1}(v)$ be the set of incoming edges to the node $v$. Due to flow constraints, we have $x[v]=\sum_{e\in \delta^{-1}(v)}x[e]$. Also for any $a,b\geq 0$, we have $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$. Hence, we have $\sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{x[v]}\leq \sum\limits_{v\in V\setminus \{\source,\sink\}}\sum\limits_{e\in\delta^{-1}(v)}\sqrt{x[e]}\leq \sum\limits_{e\in E}\sqrt{x[e]}$. The last inequality follows from the simple fact that for $v_1\neq v_2$, we have $\delta^{-1}(v_1)\cap\delta^{-1}(v_2)=\emptyset$.

\noindent
Now we have the following:
\begin{align*}
    \max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{v\in V\setminus \{\source,\sink\}}\sqrt{x[v]}+\sum\limits_{e\in E}\sqrt{x[e]}+\sum\limits_{i=1}^{K-1}\sqrt{x[\ell+i]}&\leq \max\limits_{x\in \operatorname{co}(\calX)}2\sum\limits_{e\in E}\sqrt{x[e]}+\sum\limits_{i=1}^{K-1}\sqrt{x[\ell+i]}\\
    &\leq 2\max\limits_{x\in \operatorname{co}(\calX)}2\sum\limits_{e\in E}\sqrt{x[e]}+\max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{i=1}^{K-1}\sqrt{x[\ell+i]}\\
    &\leq 3\max\limits_{x\in \operatorname{co}(\calX)}\sum\limits_{e\in E}\sqrt{x[e]} =3\calC^\star
\end{align*}

\subsection{General guarantee for sets that reduce to DAG}\label{sec:algo3-general-guarantee}
\todo[Arnab]{This section is only for pseudo-regret. Might discard it if time doesn't permit.}

Consider a combinatorial set $\calX\subseteq \{0,1\}^d$. Let $G=(V,E)$ be a DAG such that following holds:
\begin{itemize}
    \item There exists a bijective mapping between $\calX$ and the set of all paths from source to sink in $G$.
    \item Let $\bfx\in \calX$ be mapped to a path $p$. Then for any loss vector $\bfy\in \mathbb{R}^d$, there exists a loss function $\bfy^E:E\to\mathbb{R}$ such $\langle \bfx,\bfy\rangle=\sum_{e\in p }\bfy^E[e]$.
\end{itemize}

Let $\calX_{G}\subseteq\{0,1\}^{|E|}$ be the collection of all paths in $G$ indexed by the edges in $E$. Let $\calC^\star:=\max_{x\in\operatorname{co}(\calX_G)}\sum_{e\in E}\sqrt{x[e]}$. Now we claim that executing our algorithm from \Cref{sec:alg-centroid} on $G$ leads to a regret of the order of $\min\{\calC^\star\sqrt{T},\sqrt{|E|T\log |\calX|}\}$, upto to a $\log |V|$ factor. Recall that in \Cref{sec:alg-centroid} we showed that our algorithm incurs a regret of at most $\mathcal{O}(\sqrt{|E|T\log |\calX|})$, upto to a $\log |V|$ factor. Hence, it suffices to show that our algorithm also incurs a regret of at most $\mathcal{O}(\calC^\star\sqrt{T})$, upto a $\log |V|$ factor.

Recall that in \Cref{sec:alg-centroid}, we create a new DAG $G_{new}=(V_{new},E_{new})$ using the DAG $G$. Let $\calX_{G_{new}}\subseteq\{0,1\}^{|E_{new}|}$ be the collection of all paths in $G_{new}$ indexed by the edges in $E_{new}$. Due to analysis in Appendix XYZ, it easily follows that the regret we incur is upper bounded by $\calO(\calC_{new}\sqrt{T})$, where $\calC_{new}:=\max_{x\in\operatorname{co}(\calX_{G_{new}})}\sum_{e\in E_{new}}\sqrt{x[e]}$. Now we show that $\calC_{new}\leq \calO(\calC^\star\log |V|)$.

Recall that the edges in $E$ were partitioned as tree edges $E_{(h)}$ and non-tree edges $E\setminus E_{(h)}$. Recall that each edge in $E_{new}$ is either associated with a sub-path in $G$ or not associated with any edge. Recall that this association was captured with the mapping $f_e:E_{new}\to 2^E$. Exactly one edge $(u^+,v^-)$ in $E_{new}$ is associated with a non-tree edge $(u,v)$. Now we claim that at most $\log |V|$ edges is $E_{new}$ are associated with a tree edge $(u,v)$.

Recall that we constructed a centroid-based decomposition $\{T_c:c\in V\}$ using the spanning tree $T_V$ formed using $E_{(h)}$. Consider an edge $(u,v)\in E_{(h)}$. Let $S\subseteq V$ be the set of all vertices $c$ such that both $u$ and $v$ are part of the sub-tree $T_c=(V_c,E_c)$. Now observe that the edges in $E_{new}$ associated with $(u,v)$ is a subset of $\{(u^{-},c),(c,v^{+}):c\in S\}$. Next let us reindex the vertices in $S$ as $\{c_1,c_2,\ldots,c_{|S|}\}$ such that the $T_{c_j}$ is a subset of $T_{c_i}$ for any $i>j$. Due to the property of centroid-based decomposition, we have $|V_{c_{i+1}}|\leq |V_{c_i}|/2$. Hence $|S|\leq \log |V|$. Hence, at most $\log |V|$ edges in $E_{new}$ are associated with a tree edge $(u,v)$.

Recall that there was a bijective mapping $g$ from the paths $p_{new}$ from source to sink in $G_{new}$ to the paths $p$ from source to sink in $G$.  Let $\simplex_d$ denotes the $(d-1)$-dimensional probability simplex.  Now observe that a flow $\bfx\in \operatorname{co}(\calX_{G_{new}})$ is bijectively mapped to flow $\tilde \bfx \in \operatorname{co}(\calX_{G})$ as follows. As $\bfx\in \operatorname{co}(\calX_{G_{new}})$, there exists $\lambda\in \simplex_{|\calX_{G_{new}}|}$ indexed by elements of $\calX_{G_{new}}$ such that $\bfx:=\sum_{x\in \calX_{G_{new}}}\lambda[x]x$. Now $\tilde \bfx$ is defined as $\tilde \bfx=\sum_{x\in \calX_{G}}\lambda[g^{-1}(x)]x$.
 Now we have the following any edge $e_{new}$ which is not of the type $(c^-,c)$ or $(c,c^+)$:
\begin{align*}
    \bfx[e_{new}]&=\sum_{x\in \calX_{G_{new}}}\lambda[x]x[e_{new}]\\
    &=\sum_{x\in \calX_{G}}\lambda[g^{-1}(x)]g^{-1}(x)[e_{new}]\\
    &=\sum_{x\in \calX_{G}}\lambda[g^{-1}(x)]\prod_{\tilde e\in f_e(e_{new})}x[\tilde e]\\
    &\leq \sum_{x\in \calX_{G}}\lambda[g^{-1}(x)]\sum_{\tilde e\in f_e(e_{new})}x[\tilde e]\\
    &= \sum_{\tilde e\in f_e(e_{new})}\sum_{x\in \calX_{G}}\lambda[g^{-1}(x)]x[\tilde e]\\
    &= \sum_{\tilde e\in f_e(e_{new})}\tilde \bfx[\tilde e]
\end{align*}


Now we claim that $\sum_{e_{new}\in E_{new}}\sqrt{\bfx[e_{new}]}\leq 3\sum_{e\in E}\sqrt{\bfx[e]}\cdot \log |V|$. Let $\delta^-(v)$ denote the set of incoming edges to the node $v$ in $G_{new}$. First observe that for any $c\in V$, $\bfx[(c^-,c)]\leq \sum_{e\in\delta^-(c^-)}\bfx[e]$. Next observe that for any $c\in V$, $\bfx[(c,c^+)]\leq \sum_{e\in\delta^-(c)\setminus\{(c^-,c)\}}\bfx[e]+\bfx[(c^-,c)]\leq \sum_{e\in\delta^-(c)\setminus\{(c^-,c)\}}\bfx[e]+\sum_{e\in\delta^-(c^-)}\bfx[e]$. Let us define $\delta(c):=\delta^-(c^-)\cup \{\delta^-(c)\setminus\{(c^-,c)\}\}\cup \{\delta^-(c^+)\setminus\{(c,c^+)\}\}$. Now observe that the set of edges $\bar E_{new}:=E_{new}\setminus\{(c^-,c),(c,c^+):c\in V\}$ can be partitioned as $\{\delta(c)\}_{c\in V}$. Now using the inequality $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ for any $a,b\geq 0$, we have the following:
\begin{align*}
    \sum_{e_{new}\in E_{new}}\sqrt{\bfx[e_{new}]}&=\sum_{c\in V}\sum_{e_{new}\in\delta(c)}\sqrt{\bfx[e_{new}]}+\sqrt{\bfx[(c^-,c)]}+\sqrt{\bfx[(c,c^+)]}\\
    &\leq \sum_{c\in V}\sum_{e_{new}\in\delta(c)}\sqrt{\bfx[e_{new}]}+\sqrt{\sum_{e\in\delta^-(c^-)}\bfx[e]}+\sqrt{\sum_{e\in\delta^-(c)\setminus\{(c^-,c)\}}\bfx[e]+\sum_{e\in\delta^-(c^-)}\bfx[e]}\\
    &\leq 3\sum_{c\in V}\sum_{e_{new}\in\delta(c)}\sqrt{\bfx[e_{new}]}\\
    &\leq 3\sum_{c\in V}\sum_{e_{new}\in\delta(c)}\sqrt{\sum_{\tilde e\in f_e(e_{new})}\tilde \bfx[\tilde e]}\\
    &\leq 3\sum_{c\in V}\sum_{e_{new}\in\delta(c)}\sum_{\tilde e\in f_e(e_{new})}\sqrt{\tilde \bfx[\tilde e]}\\
    &= 3\sum_{c\in V}\sum_{e_{new}\in\delta(c)}\sum_{\tilde e\in E}\ind\{\tilde e \in f_e(e_{new}) \}\sqrt{\tilde \bfx[\tilde e]}\\
    &= 3\sum_{\tilde e\in E}\sqrt{\tilde \bfx[\tilde e]}\sum_{c\in V}\sum_{e_{new}\in\delta(c)}\ind\{\tilde e \in f_e(e_{new}) \}\\
    &\leq 3\sum_{\tilde e\in E}\sqrt{\tilde \bfx[\tilde e]}\cdot \log |V| \tag{as $\sum_{e_{new}\in E_{new}}\ind\{\tilde e \in f_e(e_{new}) \}\leq \log |V|$}
\end{align*}

Hence, we have $\calC_{new}\leq 3\calC^\star\log |V|$. Hence, our algorithm also incurs a regret of $\calO(\calC^*\sqrt{T})$, upto a $\log |V|$ factor.

\todo{Polish it. Maybe add a remark about the regret guarantee of \Cref{sec:alg-make-equal} at the start/end}.
\subsection{Additional instance where the pseudo-regret improves}
\todo[Arnab]{This is for pseudo-regret only. Might discard it.}
Consider an extensive form game with decision nodes $\calX=\{x^{\mathsf{r}},x^{(1)},x^{(2)},\ldots,x^{(L)}\}$, observation node $\calY=\{y\}$, and terminal nodes $\calZ=\{z^{(1,1)},z^{(1,2)},\ldots,z^{(1,M)}\}\cup\{z^{(2,1)},z^{(2,2)},\ldots,z^{(2,2L)}\}$. Let $A_{x^{\mathsf{r}}}=\{a_{x^{\mathsf{r}},1},a_{x^{\mathsf{r}},2},\ldots,a_{x^{\mathsf{r}},M+1}\}$. Let $B_y=\{b_{y,1},b_{y,2},\ldots,b_{y,L}\}$. For all $i\in \llbracket  \ell \rrbracket$, let $A_{x^{(i)}}=\{a_{x^{(i)},1},a_{x^{(i)},2}\}$. For all $i\in\llbracket  M \rrbracket $, we have $\rho_{x^{\mathsf{r}}}[a_{x^{\mathsf{r}},i}]=z^{(1,i)}$. We also have $\rho_{x^{\mathsf{r}}}[a_{x^{\mathsf{r}},M+1}]=y$. Next for all $i\in\llbracket  L \rrbracket $, we have $\rho_y[b_{y,i}]=x^{(i)}$. Next for all $i\in\llbracket  L \rrbracket $ and $j\in \{1,2\}$, we have $\rho_{x^{(i)}}[a_{x^{(i)},j}]=z^{(2,2i-2+j)}$. For this game, we have $N=2^L+M$. Hence, EXP3 will incur a regret of $\calO(\sqrt{|\calZ|T\log(N)})=\tilde\calO(\sqrt{(L^2+LM)T})$.

Recall our construction of the DAG for any given extensive form game. A pictorial representation of the DAG $G=(V,E)$ for the above game is presented in Figure XYZ. Let $\calX_{G}\subseteq\{0,1\}^{|E|}$ be the collection of all paths in $G$ indexed by the edges in $E$. Let $\calC^\star:=\max_{x\in\operatorname{co}(\calX_G)}\sum_{e\in E}\sqrt{x[e]}$. In \Cref{sec:refined-guarantees}, we showed that our FTRL approach from \Cref{sec:alg-make-equal} incurs a regret of $\calO(\calC^\star\sqrt{T})$. Now we claim that $C^\star\leq c\sqrt{L^2+M}$ where $c$ is some absolute constant.

Fix $\bfx\in\operatorname{co}(\calX_G)$. Due to flow constraints we have the following. First we have $\bfx[(x^{\mathsf{r}}_{\mathsf{s}},z^{(1,i)}_{\mathsf{s}})]=\bfx[(z^{(1,i)}_{\mathsf{s}},z^{(1,i)}_{\mathsf{t}})]=\bfx[(z^{(1,i)}_{\mathsf{s}},x^{\mathsf{r}}_{\mathsf{t}})]$ for all $i\in \llbracket  M \rrbracket$. Next we have $\bfx[(x^{\mathsf{r}}_{\mathsf{s}},y_{\mathsf{s}})]=\bfx[(y_{\mathsf{s}},x^{(1)}_{\mathsf{s}})]=\bfx[(x^{(L)}_{\mathsf{t}},y_{\mathsf{t}})]=\bfx[(x^{(i)}_{\mathsf{t}},x^{(i+1)}_{\mathsf{s}})]$ for all $i\in\llbracket  L-1 \rrbracket$. Next we have $\bfx[(x^{(i)}_{\mathsf{s}},z^{(2,2i-2+j)}_{\mathsf{s}})]=\bfx[(z^{(2,2i-2+j)}_{\mathsf{s}},z^{(2,2i-2+j)}_{\mathsf{t}})]=\bfx[(z^{(2,2i-2+j)}_{\mathsf{s}},x^{(i)}_{\mathsf{t}})]$ for all $i\in \llbracket  L \rrbracket$, $j\in \{1,2\}$. Finally, we have $\bfx[(x^{\mathsf{r}}_{\mathsf{s}},y_{\mathsf{s}})]=\sum_{j=1}^2\bfx[(x^{(i)}_{\mathsf{s}},z^{(2,2i-2+j)}_{\mathsf{s}})]$ for all $i\in \llbracket  L \rrbracket$, $j\in \{1,2\}$. Due to the last equality we also have $\sum_{j=1}^2\sqrt{\bfx[(x^{(i)}_{\mathsf{s}},z^{(2,2i-2+j)}_{\mathsf{s}})]}\leq 2\sqrt{\bfx[(x^{\mathsf{r}}_{\mathsf{s}},y_{\mathsf{s}})]}$ $i\in \llbracket  L \rrbracket$, $j\in \{1,2\}$. 

Due to the above equalities and inequalities, we have 
\[\sum_{e\in E}\sqrt{\bfx[e]}\leq c\left(\sum_{i=1}^M\sqrt{\bfx[(x^{\mathsf{r}}_{\mathsf{s}},z^{(1,i)}_{\mathsf{s}})]}+L\sqrt{\bfx[(x^{\mathsf{r}}_{\mathsf{s}},y_{\mathsf{s}})]}\right)\leq c\sqrt{L^2+M}\]
where $c$ is some absolute constant. We get the last inequality due to Cauchy-Schwartz inequality and the fact that $\sum_{i=1}^M\bfx[(x^{\mathsf{r}}_{\mathsf{s}},z^{(1,i)}_{\mathsf{s}})]+\bfx[(x^{\mathsf{r}}_{\mathsf{s}},y_{\mathsf{s}})]=1$. Hence, $C^\star\leq c\sqrt{L^2+M}$ where $c$ is some absolute constant.

\begin{figure}[h]
    \centering
    \tikzstyle{nodelbl}=[draw,fill=white,circle,inner sep=.5mm, minimum width=5.2mm]
    \DeclareDocumentCommand{\HighlightPath}{m}{
        \draw[black!12,line width=1.4mm] #1;
        \draw[line width=.4mm,shorten >=1mm] #1;
        \draw[-Latex] #1;
    }
    \DeclareDocumentCommand{\StandardPath}{m}{
        \draw[white,line width=.7mm] #1;
        \draw[-Latex] #1;
    }
    \begin{tikzpicture}[scale=1.3]
        \node[nodelbl] (x0) at (0,-1) {\tiny{$x^0$}};
        \node[nodelbl,label=center:{\tiny{$z^{1}$}}] (z01) at (1.,0.5) {};
        \node[nodelbl,label=center:{\tiny{$z^{2}$}}] (z02) at (1.,0.) {};
        \node[nodelbl,label=center:{\tiny{$z^{m}$}}] (z0m) at (1.,-1) {};
        \node[yshift=0.25em] at ($(z02)!0.5!(z0m)$) {\vdots};
        \node[nodelbl] (y) at (1.,-1.5) {\tiny{$y$}};
        \node[nodelbl] (x1) at (2,-1.) {\tiny{$x^1$}};
        \node[nodelbl] (xn) at (2,-2) {\tiny{$x^n$}};
        \node[yshift=0.25em] at ($(x1)!0.5!(xn)$) {\vdots};
        \node[nodelbl,label=center:{\tiny{$z^{11}$}}] (z11) at (2.6,-0.75) {};
        \node[nodelbl,label=center:{\tiny{$z^{12}$}}] (z12) at (2.6,-1.25) {};
        \node[nodelbl,label=center:{\tiny{$z^{n1}$}}] (zn1) at (2.6,-1.75) {};
        \node[nodelbl,label=center:{\tiny{$z^{n2}$}}] (zn2) at (2.6,-2.25) {};

        \foreach \edge in {
            (x0) -- (z01),
            (x0) -- (z02),
            (x0) -- (z0m),
            (x0) -- (y),
            (y) -- (x1),
            (y) -- (xn),
            (x1) -- (z11),
            (x1) -- (z12),
            (xn) -- (zn1),
            (xn) -- (zn2),
        } {
            \StandardPath \edge;
        }
    \end{tikzpicture} 
    $\Rightarrow$
    \begin{tikzpicture}[scale=1.3]
        \node[nodelbl] (x0s) at (0.7,0.) {\tiny{$x^0_s$}};
        \node[nodelbl] (x0t) at (6.9,0.) {\tiny{$x^0_t$}};
        \node[nodelbl,label=center:{\tiny{$z^{1}_s$}}] (z01s) at (2.7,1.25) {};
        \node[nodelbl,label=center:{\tiny{$z^{1}_t$}}] (z01t) at (4.9,1.25) {};
        \node[nodelbl,label=center:{\tiny{$z^{2}_s$}}] (z02s) at (2.7,0.75) {};
        \node[nodelbl,label=center:{\tiny{$z^{2}_t$}}] (z02t) at (4.9,0.75) {};
        \node[nodelbl,label=center:{\tiny{$z^{m}_s$}}] (z0ms) at (2.7,-0.25) {};
        \node[nodelbl,label=center:{\tiny{$z^{m}_t$}}] (z0mt) at (4.9,-0.25) {};
        \node[yshift=0.25em] at ($(z02s)!0.5!(z0ms)$) {\vdots};
        \node[yshift=0.25em] at ($(z02t)!0.5!(z0mt)$) {\vdots};
        \node[nodelbl] (ys) at (1.,-1.5) {\tiny{$y_s$}};
        \node[nodelbl] (yt) at (6.6,-1.5) {\tiny{$y_t$}};
        \node[nodelbl] (x1s) at (1.7,-1.5) {\tiny{$x^1_s$}};
        \node[nodelbl] (x1t) at (3.0,-1.5) {\tiny{$x^1_t$}};
        \node[nodelbl,label=center:{\tiny{$z^{11}_s$}}] (z11s) at (2.0,-0.9) {};
        \node[nodelbl,label=center:{\tiny{$z^{11}_t$}}] (z11t) at (2.7,-0.9) {};
        \node[nodelbl,label=center:{\tiny{$z^{12}_s$}}] (z12s) at (2.0,-2.1) {};
        \node[nodelbl,label=center:{\tiny{$z^{12}_t$}}] (z12t) at (2.7,-2.1) {};
        
        \node (zzz) at (3.8, -1.5) {\dots};

        \node[nodelbl] (xns) at (4.6,-1.5) {\tiny{$x^n_s$}};
        \node[nodelbl,label=center:{\tiny{$z^{n1}_s$}}] (zn1s) at (4.9,-0.9) {};
        \node[nodelbl,label=center:{\tiny{$z^{n1}_t$}}] (zn1t) at (5.6,-0.9) {};
        \node[nodelbl,label=center:{\tiny{$z^{n2}_s$}}] (zn2s) at (4.9,-2.1) {};
        \node[nodelbl,label=center:{\tiny{$z^{n2}_t$}}] (zn2t) at (5.6,-2.1) {};
        \node[nodelbl] (xnt) at (5.9,-1.5) {\tiny{$x^n_t$}};
        

        \foreach \edge in {
            (x0s) -- (z01s),
            (z01s) -- (z01t),
            (z01t) -- (x0t),
            (x0s) -- (z02s),
            (z02s) -- (z02t),
            (z02t) -- (x0t),
            (x0s) -- (z0ms),
            (z0ms) -- (z0mt),
            (z0mt) -- (x0t),
            (x0s) -- (ys),
            (yt) -- (x0t),
            (ys) -- (x1s),
            (x1s) -- (z11s),
            (z11s) -- (z11t),
            (z11t) -- (x1t),
            (x1s) -- (z12s),
            (z12s) -- (z12t),
            (z12t) -- (x1t),
            (x1t) -- (zzz),
            (zzz) -- (xns),
            (xns) -- (zn1s),
            (zn1s) -- (zn1t),
            (zn1t) -- (xnt),
            (xns) -- (zn2s),
            (zn2s) -- (zn2t),
            (zn2t) -- (xnt)
            (xnt) -- (yt),
        } {
            \StandardPath \edge;
        }
    \end{tikzpicture} 
    \caption{Example extensive-form game 2}
\end{figure}
